Verify then Steer: Progress Hallucination-Aware Recovery for Continuous Vision-and-Language Navigation

Vision-and-Language Navigation (VLN) requires an agent to follow language instructions to reach a target in an unseen 3D environment. However, existing methods still struggle to recover from route deviations at test time. We investigate this limitation through the lens of instruction progress, and trace it to a phenomenon we term progress hallucination: agents misinterpret off-route observations as evidence of task progress, causing their internal instruction progress to advance beyond the actual task stage and hindering recovery based on earlier sub-instructions. To address this failure mode, we propose PHAR (Progress Hallucination-Aware Recovery), a test-time recovery framework following a verify-then-steer paradigm. The verifier examines residual-stream representations of the Vision-Language Model (VLM) to identify mismatch of cross-modal evidence along the trajectories, and uses split conformal calibration to control false alarms. When an alarm is raised, the steering module uses a contextual bandit to adaptively select the rewind extent of instruction progress for online recovery. Through extensive experiments on R2R-CE and RxR-CE, our framework enhances the reliability of multiple state-of-the-art vision-language navigation methods at test time.

==> fig/teaser.tex <==
\begin{strip}
\centering
\includegraphics[width=.33\linewidth]{example-image-golden}\hfill
\includegraphics[width=.33\linewidth]{example-image-golden}\hfill
\includegraphics[width=.33\linewidth]{example-image-golden}
\captionsetup{hypcap=false}
\captionof{figure}{\textbf{Teaser} -- example of a 2-column teaser. This figure appears at the top of the first page, and a two-column teaser is not mandatory.}
\captionsetup{hypcap=true}
\label{fig:\currfilebase}%
\end{strip}
